Evaluating Structural Generalization in Neural Machine Translation

Compositional generalization refers to the ability to generalize to novel combinations of previously observed words and syntactic structures. Since it is regarded as a desired property of neural models, recent work has assessed compositional generalization in machine translation as well as semantic parsing. However, previous evaluations with machine translation have focused mostly on lexical generalization (i.e., generalization to unseen combinations of known words). Thus, it remains unclear to what extent models can translate sentences that require structural generalization (i.e., generalization to different sorts of syntactic structures). To address this question, we construct SGET, a machine translation dataset covering various types of compositional generalization with control of words and sentence structures. We evaluate neural machine translation models on SGET and show that they struggle more in structural generalization than in lexical generalization. We also find different performance trends in semantic parsing and machine translation, which indicates the importance of evaluations across various tasks.

==> sources/figure_pattern.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{sources/fig_pattern_1.png}
    \caption{List of seven categories of generalization patterns.
    Each sentence in English in the table is paired with its translation in Japanese.}
    \label{fig:pattern}
\end{figure*}


==> sources/table_generalization_examples.tex <==
    \scriptsize
    \begin{longtable}{p{12.7em}p{14.05em}p{14.2em}}
    
    \label{table:Generalization-example}\\
    \toprule
    Pattern & Training & Generalization\\
    \midrule
    \multicolumn{3}{c}{Novel Combination of Familiar Primitives and Grammatical Roles}\\
    \midrule
     Subj $\rightarrow$ Obj (common)& 
     The \textbf{goat} ate the apple. &
     The dog found the \textbf{goat}. \\
     Subj $\rightarrow$ Obj (proper)&
     \textbf{Chris} liked the woman. &
     The baby gave \textbf{Chris} the key.\\
     Obj $\rightarrow$ Subj (common) &
     The woman found the \textbf{panda}. & 
     The \textbf{panda} cleaned.\\
     Obj $\rightarrow$ Subj (proper) &
     The man liked \textbf{Taylor}. &
     \textbf{Taylor} bought Oliver the bag.\\
     Prim $\rightarrow$ Subj (common) &
     \textbf{thief}&
     The \textbf{thief} fell.\\
     Prim $\rightarrow$ Subj (proper) &
     \textbf{Coco}&
     \textbf{Coco} ate.\\
     Prim $\rightarrow$ Obj (common) &
     \textbf{trainer}&
     The friend found the \textbf{trainer}.\\
     Prim $\rightarrow$ Obj (proper) &
     \textbf{Nova}&
     A book was passed to \textbf{Nova}.\\
     Prim $\rightarrow$ Infinitive (verb) &
     \textbf{jump} &
     Mason decided to \textbf{jump}.\\
    \midrule
    \multicolumn{3}{c}{Novel Combination of Modification and Grammatical Roles}\\
    \midrule
    PP in Direct Obj &&\\
    $\rightarrow$ PP in Subj&
     The child offered \textbf{the book} \textbf{in the corner} to the princess. &
     \textbf{The book beside the bed} fell.\\ 
     $\rightarrow$ PP in Indirect Obj&
     The child offered \textbf{the book} \textbf{in the corner} to the princess.&
     The child gave a book to \textbf{the doctor in the house}.\\
    RC in Direct Obj &&\\
     $\rightarrow$ RC in Subj &
     The dog gave Liam \textbf{the apple that the dog liked}.&
     \textbf{The kid that found Emma} ate an apple.\\
     $\rightarrow$ RC in Indirect Obj &
     The dog gave Liam \textbf{the apple that the dog liked}.&
     The dog gave the apple to the kid that Liam loved.\\
    Adj in Direct Obj &&\\
     $\rightarrow$ Adj in Subj&
     The driver found \textbf{the tall girl}.&
     \textbf{The tall girl} found the driver.\\
     $\rightarrow$ Adj in Indirect Obj &
     The driver found \textbf{the tall girl}. &
     The doctor gave the book to \textbf{the tall girl}.\\
    \midrule
    \multicolumn{3}{c}{Novel Depth of Recursions}\\
    \midrule
     CC recursion shallower: \newline depth 1,2,4 $\rightarrow$ depth 3&
     The kid admired \textbf{that} Liam dreamed \textbf{that} the friend was helped by the horse.
     & Samuel believed \textbf{that} Liam thought \textbf{that} the men knew \textbf{that} the women packed the fig.\\
     CC recursion deeper: \newline depth 1,2,4 $\rightarrow$ depth 5,6 &
     The kid admired \textbf{that} Liam dreamed \textbf{that} the friend was helped by the horse. &
     A patient thought \textbf{that} Liam said \textbf{that} a tenant meant \textbf{that} a girl proved \textbf{that} Olivia wished \textbf{that} Ava ran.\\
     PP recursion shallower: \newline depth 1,2,4 $\rightarrow$ depth 3 &
     A soldier found the bottle \textbf{on the book on the table}. &
     Noah found a book \textbf{on the table in the room in the house}.\\
     PP recursion deeper: \newline depth 1,2,4 $\rightarrow$ depth 5,6&
     A soldier found the bottle \textbf{on the book on the table}. &
     Noah found a book \textbf{beside the cup on the table in the room in the house on the road}.\\
     CE recursion shallower: \newline depth 1,2,4 $\rightarrow$ depth 3 &
     A bird sought a book \textbf{that} the child \textbf{that} a mother knew found. &
     The friend found a cup \textbf{that} a monkey \textbf{that} a guy \textbf{that} the fish knew observed broke.\\
     CE recursion deeper: \newline depth 1,2,4 $\rightarrow$ depth 5,6 &
     A bird sought a book \textbf{that} the child \textbf{that} a mother knew found. &
     A girl loved a mother \textbf{that} the guy \textbf{that} the fish \textbf{that} the visitor \textbf{that} the child \textbf{that} Olivia called discovered drew heard knew.\\	
     Adj recursion shallower: \newline depth 1,2,4 $\rightarrow$ depth 3 &
     Ava bought a \textbf{rare blue} table.&
     James called the \textbf{funny tall young Japanese} friend.\\
     Adj recursion deeper: \newline depth 1,2,4 $\rightarrow$ depth 5,6 &
     Ava bought a \textbf{rare blue} table. &
     Noah noticed \textbf{the beautiful big square new red} bag.\\
    \midrule
    \multicolumn{3}{c}{Verb Argument Structure Alternation}\\
    \midrule
    Active $\rightarrow$ Passive &
    The man \textbf{moved} the car.&
    The tool was \textbf{moved}.\\
    Passive $\rightarrow$ Active &
    The apple was \textbf{dropped}.&
    The child \textbf{dropped} the book.\\
    Object-omitted transitive $\rightarrow$ transitive &
    John \textbf{wrote}.&
    The bunny \textbf{wrote} the book.\\
    Unaccusative $\rightarrow$ transitive &
    The apple \textbf{exploded}.&
    Lucy \textbf{exploded} the cup.\\
    Double Object $\rightarrow$ PP &
    John \textbf{granted} Mary the book.	&
    The teacher \textbf{granted} the plate to the child.\\
    PP $\rightarrow$ Double Object &
    John \textbf{gifted} the book to Mary.&
    Ava \textbf{gifted} the friend the chair.\\
    \midrule
    \multicolumn{3}{c}{Novel Combination of Familiar Structures}\\
    \midrule
    Subj, Direct Obj mod RC \newline $\rightarrow$ Indirect Obj mod RC &
    The director knows the guy that the child liked. / 
    Liam knows a kid that gave the teacher a pen. &
    The visitor liked the guy that the friend gave the plant to.\\
    Subj, Direct Obj wh-question \newline $\rightarrow$ Indirect Obj wh-question &
    Who appreciated the book? /
    Who did Liam call? &
    Who did Liam give a shoe to?\\
    \midrule
    \multicolumn{3}{c}{Novel Structure of wh-questions}\\
    \midrule
    Transitive&&\\
    $\rightarrow$ Active Subject &
    Who broke the cup? &
    Who wanted to talk?\\
    $\rightarrow$ Passive Subject &
    Who broke the cup?&
    What is broken?\\
    $\rightarrow$ Direct Obj, Ditransitive &
    What did the girl break?&
    What did the girl give to the boy?\\
    $\rightarrow$ Subject with PP &
    What did the girl break?&
    What did the boy in the car eat?\\
    $\rightarrow$ Long movement &
    What did the girl break?&
    What did the teacher think that the girl break?\\
    \midrule
    \multicolumn{3}{c}{Novel Tense}\\
    \midrule
    Past &&\\
    $\rightarrow$ Present (Ditransitive) &
    Ava \textbf{returned} the doll to Lucas. &
    Olivia \textbf{returns} a box to the kid.\\
    $\rightarrow$ Present (Infinitive) &
    A child \textbf{wanted} to run. &
    A child \textbf{wants} to talk.\\
    $\rightarrow$ Present (Complement) &
    The host \textbf{hoped} that Noah grew. &
    A hero \textbf{hopes} that Olivia was helped.\\
    Past, Present (transitive) &&\\
    $\rightarrow$ Present (Ditransitive) &
    The friend \textbf{showed} a guitar. / Theodore \textbf{showed} the book to the mother. / The friend \textbf{shows} a big bowl.&
    A patient \textbf{shows} the father a cup.\\
    $\rightarrow$ Present (Infinitive) &
    The child \textbf{prepared} a cup. / A boy \textbf{prepared} to walk. / The guest \textbf{prepares} the box.&
    The mother \textbf{prepares} to talk.\\
    $\rightarrow$ Present (Complement) &
    A child \textbf{learned} the newspaper. / Emma \textbf{learned} that a shoe broke. / A student \textbf{learns} a book.&
    A girl \textbf{learns} that the cup was found.\\
    \bottomrule
    \caption[List of generalization patterns.]{List of generalization patterns. Subj represents subject, Obj represents object, Prim represents primitive, mod represents modification, CP represents complement clause, PP represents prepositional phrase, CE represents center-embedding, Adj represents adjective.}
    
    \end{longtable}
    \normalsize


==> sources/table_pattern_combination.tex <==
\begin{table*}[t]
    \centering
    
    \footnotesize
    \begin{tabular}{p{0.31\linewidth}p{0.29\linewidth}p{0.31\linewidth}}
    \toprule
    Pattern & Training & Generalization \\
    \midrule
    Subj, Direct Obj extracted RC \newline $\rightarrow$ Indirect Obj extracted RC &
    The director knew \textbf{the guy that the child liked}. / 
    Liam knew \textbf{a kid that gave the teacher a pen}. &
    The visitor liked \textbf{the guy that the friend gave the plant to}.\\
    Subj, Direct Obj extracted wh-question \newline $\rightarrow$ Indirect Obj extracted wh-question &
    \textbf{Who appreciated} the book? /
    \textbf{Who} did Liam \textbf{call}? &
    \textbf{Who} did Liam \textbf{give} a shoe \textbf{to}?\\
     \bottomrule
    \end{tabular}
    \caption[List of patterns in novel combination of familiar structures.]{List of patterns in novel combination of familiar structures.}
    \label{table:pattern_combination}
\end{table*}


==> sources/table_pattern_modified.tex <==
\begin{table}[t]
    \centering
    
    \footnotesize
    \begin{tabular}{p{0.27\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
    \toprule
    Pattern & Training & Generalization \\
    \midrule
    PP in Direct Obj &&\\
    $\rightarrow$ PP in Subj&
     The child gave \textbf{the pen on the table} to Liam. &
     \textbf{The book beside the bed} fell.\\ 
     $\rightarrow$ PP in Indirect Obj&
     The child gave \textbf{the pen on the table} to Liam.&
     The child gave a book to \textbf{the doctor in the house}.\\
    RC in Direct Obj &&\\
     $\rightarrow$ RC in Subj &
     The dog gave Liam \textbf{the apple that the dog liked}.&
     \textbf{The kid that found Emma} ate an apple.\\
     $\rightarrow$ RC in Indirect Obj &
     The dog gave Liam \textbf{the apple that the dog liked}.&
     The dog gave the apple to the kid that Liam loved.\\
    Adj in Direct Obj &&\\
     $\rightarrow$ Adj in Subj&
     The driver found \textbf{the tall girl}.&
     \textbf{The tall girl} found the driver.\\
     $\rightarrow$ Adj in Indirect Obj &
     The driver found \textbf{the tall girl}. &
     The doctor gave the book to \textbf{the tall girl}.\\
     \bottomrule
    \end{tabular}
    \caption[List of patterns in novel combination of modification and grammatical roles.]{List of patterns in novel combination of modification and grammatical roles.}
    \label{table:pattern_modified}
\end{table}


==> sources/table_pattern_primitive.tex <==
\begin{table*}[t]
    \centering
    
    \footnotesize
    \begin{tabular}{p{0.27\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
    \toprule
    Pattern & Training & Generalization \\
    \midrule
    Subj $\rightarrow$ Obj (common)& 
     The \textbf{goat} ate the apple. &
     The dog found the \textbf{goat}. \\
     Subj $\rightarrow$ Obj (proper)&
     \textbf{Chris} liked the woman. &
     The baby gave \textbf{Chris} the key.\\
     Obj $\rightarrow$ Subj (common) &
     The woman found the \textbf{panda}. & 
     The \textbf{panda} ran.\\
     Obj $\rightarrow$ Subj (proper) &
     The man liked \textbf{Taylor}. &
     \textbf{Taylor} bought Oliver the bag.\\
     Prim $\rightarrow$ Subj (common) &
     \textbf{thief}&
     The \textbf{thief} fell.\\
     Prim $\rightarrow$ Subj (proper) &
     \textbf{Coco}&
     \textbf{Coco} ate.\\
     Prim $\rightarrow$ Obj (common) &
     \textbf{trainer}&
     The friend found the \textbf{trainer}.\\
     Prim $\rightarrow$ Obj (proper) &
     \textbf{Nova}&
     A book was passed to \textbf{Nova}.\\
     Prim $\rightarrow$ Infinitive (verb) &
     \textbf{jump} &
     Mason decided to \textbf{jump}.\\
     \bottomrule
     
    \end{tabular}
    \caption[List of patterns in primitive substitution.]{List of patterns in primitive substitution.}
    \label{table:pattern_primitive}
\end{table*}


==> sources/table_pattern_question.tex <==
\begin{table*}[t]
    \centering
    
    \footnotesize
    \begin{tabular}{p{0.28\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
    \toprule
    Pattern & Training & Generalization \\
    \midrule
    Transitive&&\\
    $\rightarrow$ Active Subject &
    \textbf{Who broke} the cup? &
    \textbf{Who wanted} to talk?\\
    $\rightarrow$ Passive Subject &
    \textbf{Who broke} the cup?&
    \textbf{What was broken}?\\
    $\rightarrow$ Direct Obj, Ditransitive &
    \textbf{What} did the girl \textbf{break}?&
    \textbf{What} did the girl \textbf{give} to the boy?\\
    $\rightarrow$ Subject with PP &
    What did \textbf{the girl} break?&
    What did \textbf{the boy in the car} eat?\\
    $\rightarrow$ Long movement &
    \textbf{What} did the girl \textbf{break}?&
    \textbf{What} did the teacher think that the girl \textbf{break}?\\
     \bottomrule
    \end{tabular}
    \caption[List of patterns in novel structure of \textit{wh}-questions.]{List of patterns in novel structure of \textit{wh}-questions.}
    \label{table:pattern_question}
\end{table*}


==> sources/table_pattern_recursion.tex <==
\begin{table*}[t]
    \centering
    
    \footnotesize
    \begin{tabular}{p{0.29\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
    \toprule
    Pattern & Training & Generalization \\
    \midrule
     Adj recursion shallower: \newline depth 1, 2, 4 $\rightarrow$ depth 3 &
     Ava bought a \textbf{rare blue} table.&
     James called the \textbf{funny tall young} friend.\\
     Adj recursion deeper: \newline depth 1, 2, 4 $\rightarrow$ depth 5, 6 &
     Ava bought a \textbf{rare blue} table. &
     Noah noticed \textbf{the beautiful big square new red} bag.\\
     \bottomrule
    \end{tabular}
    \caption[List of patterns in novel depth of recursions.]{List of patterns in novel depth of recursions.}
    \label{table:pattern_recursion}
\end{table*}


==> sources/table_pattern_tense.tex <==
\begin{table*}[t]
    \centering
    
    \footnotesize
    \begin{tabular}{p{0.27\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
    \toprule
    Pattern & Training & Generalization \\
    \midrule
    Past &&\\
    $\rightarrow$ Present (Ditransitive) &
    Ava \textbf{lent} the doll to Lucas. &
    Olivia \textbf{lends} a box to the kid.\\
    $\rightarrow$ Present (Infinitive) &
    A child \textbf{wanted} to run. &
    A child \textbf{wants} to talk.\\
    $\rightarrow$ Present (Complement) &
    The host \textbf{hoped} that Noah grew. &
    A hero \textbf{hopes} that Olivia was helped.\\
    \midrule
    Past, Present (Transitive) &&\\
    $\rightarrow$ Present (Ditransitive) &
    The friend \textbf{showed} a guitar. / Theodore \textbf{showed} the book to the mother. / The friend \textbf{shows} a big bowl.&
    A patient \textbf{shows} the father a cup.\\
    $\rightarrow$ Present (Infinitive) &
    The child \textbf{prepared} a cup. / A boy \textbf{prepared} to walk. / The guest \textbf{prepares} the box.&
    The mother \textbf{prepares} to talk.\\
    $\rightarrow$ Present (Complement) &
    A child \textbf{learned} the newspaper. / Emma \textbf{learned} that a shoe broke. / A student \textbf{learns} a book.&
    A girl \textbf{learns} that the cup was found.\\
     \bottomrule
     
    \end{tabular}
    \caption[List of patterns in novel tense.]{List of patterns in novel tense.}
    \label{table:pattern_tense}
\end{table*}


==> sources/table_pattern_verb.tex <==
\begin{table*}[t]
    \centering
    
    \footnotesize
    \begin{tabular}{p{0.28\linewidth}p{0.32\linewidth}p{0.31\linewidth}}
    \toprule
    Pattern & Training & Generalization \\
    \midrule
    Active $\rightarrow$ Passive &
    The man \textbf{moved} the car.&
    The tool was \textbf{moved}.\\
    Passive $\rightarrow$ Active &
    The apple was \textbf{dropped}.&
    The child \textbf{dropped} the book.\\
    Object-omitted Transitive $\rightarrow$ Transitive &
    John \textbf{wrote}.&
    The bunny \textbf{wrote} the book.\\
    Unaccusative $\rightarrow$ Transitive &
    The apple \textbf{exploded}.&
    Lucy \textbf{exploded} the ball.\\
    Double Object $\rightarrow$ PP &
    John \textbf{granted} Mary the book.	&
    The teacher \textbf{granted} the plate to the child.\\
    PP $\rightarrow$ Double Object &
    John \textbf{gifted} the book to Mary.&
    Ava \textbf{gifted} the friend the chair.\\
     \bottomrule
    \end{tabular}
    \caption[List of patterns in verb argument structure alternation.]{List of patterns in verb argument structure alternation.}
    \label{table:pattern_verb}
\end{table*}

